Attacks, Defenses, And Tools: A Framework To Facilitate Robust AI/ML Systems

Software systems are increasingly relying on Artificial Intelligence (AI) and Machine Learning (ML) components. The emerging popularity of AI techniques in various application domains attracts malicious actors and adversaries. Therefore, the developers of AI-enabled software systems need to take into account various novel cyber-attacks and vulnerabilities that these systems may be susceptible to. This paper presents a framework to characterize attacks and weaknesses associated with AI-enabled systems and provide mitigation techniques and defense strategies. This framework aims to support software designers in taking proactive measures in developing AI-enabled software, understanding the attack surface of such systems, and developing products that are resilient to various emerging attacks associated with ML. The developed framework covers a broad spectrum of attacks, mitigation techniques, and defensive and offensive tools. In this paper, we demonstrate the framework architecture and its major components, describe their attributes, and discuss the long-term goals of this research.

==> sections/implementation.tex <==
%\section{Implementation} \label{sec:implementation}
\subsection{Implementation} \label{sec:implementation}


% To fully comprehend the existing problems in AI/ML and provide appropriate mitigation techniques, we considered their behavior, impact on the system, their attributes, and their goal. 
 
% As a result of this research, we developed an interactive online framework. This framework supports researchers and developers in identifying and understanding the potential threats against AI/ML systems and their relationship. It allows users to apply multiple filters to focus on the problem and view them as they want, get into details as much as necessitated, and find the best potential solutions to tackle the problem, considering the advantages, disadvantages, and the solutions' side effects. 
